Towards Cohesion-Fairness Harmony: Contrastive Regularization in Individual Fair Graph Clustering

Conventional fair graph clustering methods face two primary challenges: i) They prioritize balanced clusters at the expense of cluster cohesion by imposing rigid constraints, ii) Existing methods of both individual and group-level fairness in graph partitioning mostly rely on eigen decompositions and thus, generally lack interpretability. To address these issues, we propose iFairNMTF, an individual Fairness Nonnegative Matrix Tri-Factorization model with contrastive fairness regularization that achieves balanced and cohesive clusters. By introducing fairness regularization, our model allows for customizable accuracy-fairness trade-offs, thereby enhancing user autonomy without compromising the interpretability provided by nonnegative matrix tri-factorization. Experimental evaluations on real and synthetic datasets demonstrate the superior flexibility of iFairNMTF in achieving fairness and clustering performance.

==> Extended_Related_Works.tex <==
\subsection{What Is Individual Fairness?}
The initial definition of individual fairness/bias was first introduced as an abstract definition, regardless of the type of input data, in \cite{DBLP:conf/innovations/DworkHPRZ12} which states that a model $f$ is fair if, for any pair of inputs $x, x'$ which are sufficiently close (as per an appropriate metric), the model outputs $f(x), f(x')$ are also close (as per another appropriate metric). In other terms, a model is fair if, any pair of similar individuals in the input space receive also similar treatments (predictions) in the output space $(i.e., f(x) = f(x'))$. For regression models, this means that the absolute difference $|f(x)-f(x')|$ is sufficiently small.

according to \cite{DBLP:conf/uai/JohnVS20}, in the regression perspective, if $f : \mathbb{R}^r \rightarrow \mathbb{R}$ is a decision model with $r$ being the number of features, the abstract definition of individual fairness, given by \cite{DBLP:conf/innovations/DworkHPRZ12}, is as follows: Given appropriate distance functions — $d(\cdot, \cdot)$ on $\mathbb{R}^d$ (the domain of $f$) and $D(\cdot, \cdot)$ on $\mathbb{R}$ (the co-domain of $f$) — as well as thresholds $\epsilon \geq 0$ and $\delta \geq 0$, the model is individually fair if, for any pair of inputs $x, x'$ such that $d(x, x') \leq \epsilon$, we have $D(f(x), f(x')) \leq \delta$.

\subsection{Individual Fairness in Graph Mining}
In  \cite{dong2023fairness} a comprehensive taxonomy of individual fairness has also been studied from a graph mining perspective. According to their definition, individual fairness does not consider any sensitive features. Instead, it focuses on fairness at the individual (e.g., each node in graph data) level. Based on this definition, individual fairness requires that similar individuals should be treated similarly. Hence, it is considered as a fairness notion at a finer granularity than group fairness. In this paper, individual fairness is divided into three categories based on different graph mining applications: 1- Node Pair Distance-Based Fairness, 2- Node Ranking-Based Fairness, and 3- Individual Fairness in Graph Clustering. 
The first group of notions notion extend the individual fairness of \cite{DBLP:conf/innovations/DworkHPRZ12}, which is based on the idea that pair-wise node distances in the input space and output space should satisfy Lipschitz Condition. Specifically, Lipschitz condition requires that the distance of any node pairs in the output space should be smaller or equal to their corresponding distance in the input space (usually re-scaled by a scalar). Formally, given a pair of nodes $v_i$ and $v_j$, Lipschitz condition is given as 

\begin{equation}
    D(f(v_i), f(v_j)) \leq L \cdot d(v_i, v_j)
\end{equation}
where $f(\cdot)$is the predictive model that gives the node level output (e.g., node embeddings). $D(\cdot, \cdot)$ and $d(\cdot, \cdot)$ are the distance metrics in the output and input space, respectively. $L$ is the Lipschitz constant that re-scales the input distance between node $v_i$ and
$v_j$. To measure individual fairness based on Lipschitz condition, \cite{DBLP:conf/icml/ZemelWSPD13} proposed Consistency on non-graph data with the intuition to measure the average distance of the output between each individual and its k-nearest neighbors such that:

\begin{equation}
    1-\frac{1}{n\cdot k}\sum^{i=1}_{n}\Big|f(x_i)-\sum_{j\in kNN(x_i)}f(x_j)\Big|
\end{equation}
where $f(x_i)$ is the probabilistic classification output for node features $x_i$ of node $v_i$, function $kNN$ takes the features of node $v_i$ as input and returns the index set of its k-nearest neighbors in the feature space. In general, a larger average distance indicates a lower level of individual
fairness. 

In graph mining algorithms, a similar formulation of consistency is proposed by \cite{DBLP:journals/pvldb/LahotiGW19} based on similarity matrix $S$. Generally, $S$ describes the similarity between nodes in the input space and can be given based on attributes, graph topology, or knowledge from domain experts. Here, consistency is formulated as: 
\begin{equation}
    1-\frac{\sum_{i}\sum_{j}|f(x_i)-f(x_j)|\cdot S_{ij}}{\sum_{i}\sum_{j}S_{ij}}, \quad (i\neq j)
\end{equation}
in binary node classification tasks. For any graph mining algorithm, a large value of consistency indicates that it gives similar outputs for similar nodes in the input space, i.e., the algorithm performs well on individual fairness. 
Moreover, in \cite{DBLP:conf/kdd/KangHMT20} a measure is proposed that calculates the similarity-weighted output discrepancy between nodes to measure unfairness, which is formulated as $Tr(H^\top L_S H)$ where $L_S$ denotes the Laplacian matrix of the similarity matrix $S$ and
$H \in \mathbb{R}^{n\times k}$ is the output matrix of the graph mining algorithm. Each row in $H$ represents the output vector for on of the $n$ corresponding nodes and $Tr(\cdot)$ is the trace operator for any matrix. This metric measures the weighted sum of pair-wise node distance in the output space, where the weighting score is the pair-wise node similarity. Hence for any graph mining algorithms, a smaller
value of the similarity-weighted discrepancy typically implies a
higher level of individual fairness.

Category 2 is based on node rankings as introduced in \cite{DBLP:conf/kdd/DongKTL21}: given a pair-wise similarity matrix $S$ of individuals in the input space, each individual has a ranking list $R_1$ that indicates the relative similarity ranking between itself and others. Similarly, a corresponding ranking list $R_2$ can also be derived based on the pair-wise individual similarity in the output space. From the perspective of node ranking, individual fairness is regarded as fulfilled when the two ranking lists ($R_1$ and $R_2$) are the same for each individual.

The third category surveys an individual fairness measure for Graph Clustering based on the definition in \cite{DBLP:conf/nips/GuptaD22}. In clustering, the criterion of individual fairness is defined in a different way compared with other tasks. Specifically, for each node in a graph, if its neighbors are proportionally distributed to each cluster, individual fairness is then fulfilled \cite{DBLP:journals/corr/abs-2105-03714}. Formally, a clustering algorithm satisfies individually fair clustering for node $v_i$ if
\begin{equation}
    \frac{|\{v_j: \bm{A}_{i,j}=1 \land v_j \in C_k\}|}{|C_k|} = \frac{|\{v_j: \bm{A}_{i,j}=1|}{|V|}
\end{equation}
for all $k \in \{1,\ldots, K\}$. Here $K$ is the total number of clusters, and $C_k$ represents the set of nodes in cluster $k$. The intuition is that for each node, the ratio occupied by its one-hop neighbors in each cluster should be the same as the ratio occupied by its one-hop neighbors in the population. We then introduce the metric to quantify fair clustering. Specifically, $\rho_i$ measures how disproportionately the one-hop neighbors of node $v_i$ are assigned in different clusters. Formally, $\rho_i$ is defined as:  
\begin{equation}
    \rho_i = min_{k,l\in \{1,\ldots,K\}} \frac{|C_k: \cap N_{v_i} |} {|C_l: \cap N_{v_i}|}
\end{equation}
where $N_{v_i}$ denotes the neighboring node set of $v_i$. In \cite{DBLP:journals/corr/abs-2105-03714}, the average $\rho_i$ across all nodes in the graph is employed as the metric of individual fairness in graph clustering.
